POLY-HOOT: Monte-Carlo Planning in Continuous Space MDPs with Non-Asymptotic Analysis

Monte-Carlo planning, as exemplified by Monte-Carlo Tree Search (MCTS), has demonstrated remarkable performance in applications with finite spaces. In this paper, we consider Monte-Carlo planning in an environment with continuous state-action spaces, a much less understood problem with important applications in control and robotics. We introduce POLY-HOOT, an algorithm that augments MCTS with a continuous armed bandit strategy named Hierarchical Optimistic Optimization (HOO) (Bubeck et al., 2011). Specifically, we enhance HOO by using an appropriate polynomial, rather than logarithmic, bonus term in the upper confidence bounds. Such a polynomial bonus is motivated by its empirical successes in AlphaGo Zero (Silver et al., 2017b), as well as its significant role in achieving theoretical guarantees of finite space MCTS (Shah et al., 2019). We investigate, for the first time, the regret of the enhanced HOO algorithm in non-stationary bandit problems. Using this result as a building block, we establish non-asymptotic convergence guarantees for POLY-HOOT: the value estimate converges to an arbitrarily small neighborhood of the optimal value function at a polynomial rate. We further provide experimental results that corroborate our theoretical findings.

==> 2preliminaries_0.tex <==

\section{Preliminaries}\label{sec:preliminaries}
 
\subsection{Markov Decision Processes}
An MDP can be represented by a 5-tuple $(S, A, T, R, \gamma)$,  where $S\subseteq \rr^n$ is the continuous state space, $A\subseteq \rr^m$ the continuous action space, $T:S\times A \ra S$ the deterministic transition function, $R:S\times A\ra \rr$ the stochastic reward function, and $\gamma \in (0,1)$ is the discount factor. We do not require $S$ and $A$ to be compact, thus our theory covers many control applications with possibly unbounded state-action spaces. We assume the reward function is bounded, i.e., there exists a constant $R_{max}>0$ such that $0\leq R(s,a)\leq R_{max},\forall s\in S,a\in A$. Note that we assume the state transitions to be deterministic. This is a common setting in the MCTS literature~\citep{browne2012survey,shah2019reinforcement,kimmonte}, as MCTS was historically introduced and popularly utilized in problems like Go~\citep{gelly2006modification,silver2017mastering} and Atari games~\citep{guo2014deep}, where the state transitions are inherently deterministic. For simplicity we use the notation $ s\circ a \triangleq T(s,a) $ to denote the next state deterministically reached by taking action $a\in A$ at the current state $s\in S$. 

A policy $\pi:S\ra A$ specifies the action $ a=\pi(s) $ taken at state $ s $. The value function $V^\pi:S\ra \rr$ of a policy $\pi$ is defined as the expected discounted sum of rewards following the policy $\pi$ starting from the current state $s\in S$, i.e., $V^{\pi}(s)=\mathbb{E}_{\pi}\left[\sum_{t=0}^{\infty} \gamma^{t} R\left(s_{t}, a_{t}\right) | s_{0}=s\right]$. Similarly, define the state-action value function $Q^{\pi}(s,a)=\mathbb{E}_{\pi}\left[\sum_{t=0}^{\infty} \gamma^{t} R\left(s_{t}, a_{t}\right) | s_{0}=s, a_0 = a\right]$. The goal of the agent is to find an optimal policy $\pi^*$ that achieves the optimal value $ V^{\pi^*}(s) = V^*(s) \triangleq \sup_\pi V^\pi(s)$ for all $s\in S$.  

\subsection{Monte-Carlo Tree Search}
Monte-Carlo tree search solves a planning problem by rollout-based lookahead sampling, under the assumption that a generative model of the environment is available. One representative instance is the UCT algorithm~\citep{kocsis2006bandit}. It builds a tree of alternating state nodes and state-action nodes on different levels, and the root node is the state where planning is initiated. The value of a state-action node is the average reward over samples that have taken the given action at the corresponding state, and the value of a state node is defined as the maximum value over its child state-action nodes. At each state node, an action is chosen by following the recommendation of a UCB1~\citep{auer2002finite} bandit algorithm. {The UCB1 agent records the empirical average reward of each candidate action as well as the number of times that each action has been taken. It hence makes a trade-off between exploiting the current best action and exploring potentially better actions. In this sense, UCT can quickly rule out a large set of suboptimal actions and concentrate on the sequences of actions that potentially lead to the optimal performance. However, UCT only applies to discrete actions spaces, as the underlying UCB1 algorithm is designed for finite-armed bandit problems. }

{A major challenge in the theoretical analysis of any MCTS algorithm is the non-stationarity of bandit rewards. Since the policies at the lower level bandits of MCTS is constantly changing, the reward sequences for each bandit agent is drifting over time, causing the reward distribution to be highly non-stationary. The performance of each bandit depends on the results of a chain of bandits in the lower levels, and this hierarchical inter-dependence of bandits makes the analysis highly non-trivial. \cite{kocsis2006bandit} attempted to address this issue, but their assumption on the exponential concentration of rewards is still not very convincing. A complete solution was not provided until very recently in~\cite{shah2019reinforcement}, where the authors inductively show the polynomial concentration of rewards by leveraging a non-stationary bandit algorithm with a \emph{polynomial} bonus term. Our approach in the continuous case is based upon a similar reasoning as in~\cite{shah2019reinforcement}. }



\subsection{Hierarchical Optimistic Optimization}

HOO~\citep{bubeck2011x} is an extension of finite-armed bandit algorithms to problems with an arbitrary measurable space of arms, including those with a continuum of actions in the Euclidean space. HOO incrementally builds a binary tree covering to represent the continuous action space $X$. Each node in the HOO tree covers a subset of $X$, and this subset is further divided into two corresponding to the two child nodes. HOO selects an action by following a path from the root node to a leaf node. At each node, it chooses the child node that has the largest $B$-value, a value that makes a trade-off between exploration and exploitation to be defined later. At a leaf node, HOO randomly samples an action from the set represented by this node, and adds two child nodes to this leaf node by further decomposing the represented set into two subsets. In this manner, HOO adaptively subdivides the action space and quickly focuses on the area where potentially optimal actions lie in. 

Following the notations in~\cite{bubeck2011x}, we index the nodes in the {binary tree covering of HOO} 
by pairs of integers $(h,i)$\footnote{We use $h$ and $H$ to index the depth in the HOO tree, and use $d$ and $D$ to index the depth in the MCTS tree.}, where $h\geq 0$ denotes the depth of the node, and $1\leq i\leq 2^h$ denotes its index on depth $h$. By convention, $(0,1)$ indexes the root of the binary tree, and the two children of $(h,i)$ are denoted by $(h+1,2i-1)$ and $(h+1,2i)$. Let $\mc{P}_{h,i}\subseteq X$ be the domain covered by the node $(h,i)$, and by definition $\mc{P}_{0,1} = X$, and $
\mathcal{P}_{h, i}=\mathcal{P}_{h+1,2 i-1} \cup \mathcal{P}_{h+1, 2 i}
,\forall  h \geq 0 \text { and } 1 \leq  i \leq 2^{h}$. It can be seen that the descendants of a node $(h,i)$ lie in the subset of its domain. Let $\mc{C}(h,i)$ denotes the set of all descendants of node $(h,i)$, and let $(H_t,I_t)$ denote the node played by HOO at round $t$. Then the number of times that a descendant of $(h,i)$ has been played up to and including round $n$ is denoted by $T_{h, i}(n)=\sum_{t=1}^{n} \indicator_{\left\{\left(H_{t}, I_{t}\right) \in \mathcal{C}(h, i)\right\}},$ and the empirical average of rewards is defined as $\widehat{\mu}_{h, i}(n)=\frac{1}{T_{h, i}(n)} \sum_{t=1}^{n} Y_{t} \indicator_{\left\{\left(H_{t}, I_{t}\right) \in \mathcal{C}(h, i)\right\}}.$ In the original HOO algorithm~\citep{bubeck2011x}, the upper confidence bound of a node $(h,i)$ is defined with a logarithmic bonus term: 
\begin{equation}\label{eqn:upperconfidence}
U_{h, i}(n)=\left\{\begin{array}{ll}\widehat{\mu}_{h, i}(n)+ \sqrt{\frac{2\ln n}{T_{h,i}(n)}} +\nu_{1} \rho^{h}, & \text { if } T_{h, i}(n)>0, \\ \infty, & \text { otherwise ,}\end{array}\right.
\end{equation} 
where $\nu_1$ and $\rho$ are two constants that upper bound the maximum variation of the mean-payoff function within the domain of $\mc{P}_{h,i}$. 
